Density of the set of probability measures with the martingale representation property

Let $\psi$ be a multi-dimensional random variable. We show that the set of probability measures $\mathbb{Q}$ such that the $\mathbb{Q}$-martingale $S^{\mathbb{Q}}_t=\mathbb{E}^{\mathbb{Q}}\left[\psi\lvert\mathcal{F}_{t}\right]$ has the Martingale Representation Property (MRP) is either empty or dense in $\mathcal{L}_\infty$-norm. The proof is based on a related result involving analytic fields of terminal conditions $(\psi(x))_{x\in U}$ and probability measures $(\mathbb{Q}(x))_{x\in U}$ over an open set $U$. Namely, we show that the set of points $x\in U$ such that $S_t(x) = \mathbb{E}^{\mathbb{Q}(x)}\left[\psi(x)\lvert\mathcal{F}_{t}\right]$ does not have the MRP, either coincides with $U$ or has Lebesgue measure zero. Our study is motivated by the problem of endogenous completeness in financial economics.

==> style.tex <==
% Packages

\usepackage{amsthm} \usepackage{amsmath} \usepackage{amsfonts}
\usepackage{amssymb} \usepackage{latexsym} \usepackage{enumerate}
\usepackage{mathrsfs}
\usepackage[numbers]{natbib}
\usepackage[colorinlistoftodos, textwidth=4cm, shadow]{todonotes}

\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

% Theorems and similar

\theoremstyle{plain}%
\newtheorem{Theorem}{Theorem}[section] %
\newtheorem{Corollary}[Theorem]{Corollary}%
\newtheorem{Lemma}[Theorem]{Lemma} %
\newtheorem{Proposition}[Theorem]{Proposition} %

\theoremstyle{definition}%
\newtheorem{Assumption}[Theorem]{Assumption}%
\newtheorem{Definition}[Theorem]{Definition}%
\newtheorem{Example}[Theorem]{Example} %

\theoremstyle{remark}%
\newtheorem{Remark}[Theorem]{Remark} %

% Useful commands

\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\braces}[1]{\left\lbrace{#1}\right\rbrace}
\newcommand{\descr}[2]{\left\lbrace{#1}:\; #2 \right\rbrace}
\newcommand{\diag}[1]{\mathrm{diag}(#1)}
% Various
\newcommand{\seq}[1]{$\left(#1^n\right)_{n\geq 1}$}
\newcommand{\set}{\triangleq}
\newcommand{\supp}[1]{\sigma_{#1}}
\newcommand{\ip}[2]{\left\langle
    #1,#2 \right\rangle}
\newcommand{\pvar}[1]{\left\langle
    #1\right\rangle}
\newcommand{\pcov}[2]{\left\langle
    #1,#2 \right\rangle}
\newcommand{\qvar}[1]{\left[#1\right]}
\newcommand{\qcov}[2]{\left[
    #1,#2 \right]}
\newcommand{\idvec}{\mathbf{1}}
\newcommand{\ind}[1]{1_{\braces{#1}}}
\newcommand{\setind}[1]{1_{#1}}
\newcommand{\cind}[1]{\delta_{#1}}
\newcommand{\map}[3]{#1:\; #2 \rightarrow #3} %1=name, 2=arg_domain, 3=val_domain
\newcommand{\norm}[1]{\lVert#1\rVert} %
\newcommand{\real}[1]{\mathbb{R}^{#1}}



% Conditional expectation: measure, time, RV
\newcommand{\mM}[2]{#1\left[#2\right]}
\newcommand{\mE}[2]{\mathbb{E}^{#1}\left[#2\right]}
\newcommand{\cE}[3]{\mathbb{E}^{#1}\left[\left.#3\right\lvert\mathcal{F}_{#2}\right]} 
\newcommand{\E}[2]{\mathbb{E}^{#1}\left[#2\right]} 
\newcommand{\EP}[1]{\E{}{#1}}
\newcommand{\cEP}[2]{\cE{}{#1}{#2}}
\newcommand{\Prob}[2]{\mathbb{#1}\left[#2\right]} 
\newcommand{\ProbP}[1]{\Prob{\mathbb{P}}{#1}}

% Spaces
\newcommand{\sSpace}[2]{{{#1}_{#2}}}
\newcommand{\sNorm}[2]{\norm{#1}_{#2}}
\newcommand{\sH}[1]{{\sSpace{\mathcal{H}}{#1}}}
\newcommand{\sA}{\mathcal{A}}
\newcommand{\bmo}{\mathrm{BMO}}

% Operators


% Mathematical operators

\DeclareMathOperator*{\argmax}{arg\:max}
\DeclareMathOperator*{\argmin}{arg\:min}
\DeclareMathOperator{\boundary}{\partial}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\closure}{cl}
\DeclareMathOperator{\cov}{Cov}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\esssup}{ess\;sup}
\DeclareMathOperator*{\interior}{int}
\DeclareMathOperator*{\ri}{ri}
\DeclareMathOperator*{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\sprt}{supp}
\DeclareMathOperator{\spn}{span}



% Environments

\newcommand{\envspace}{\vspace{2mm}}
\newenvironment{ToDo}{\envspace
  \noindent {\textbf{Things to do:}}  \sf}{\envspace}
\newenvironment{ToThink}{\newline
  \noindent {\textbf{Note:}}  \sf}{\envspace}



